Object-aware Feature Aggregation for Video Object Detection

We present an Object-aware Feature Aggregation (OFA) module for video object detection (VID). Our approach is motivated by the intriguing property that video-level object-aware knowledge can be employed as a powerful semantic prior to help object recognition. As a consequence, augmenting features with such prior knowledge can effectively improve the classification and localization performance. To make features get access to more content about the whole video, we first capture the object-aware knowledge of proposals and incorporate such knowledge with the well-established pair-wise contexts. With extensive experimental results on the ImageNet VID dataset, our approach demonstrates the effectiveness of object-aware knowledge with the superior performance of 83.93% and 86.09% mAP with ResNet-101 and ResNeXt-101, respectively. When further equipped with Sequence DIoU NMS, we obtain the best-reported mAP of 85.07% and 86.88% upon the paper submitted. The code to reproduce our results will be released after acceptance.

==> intro_bk_98.tex <==
\section{Introduction}
\label{Introduction}
Convolutional neural networks~(CNNs)~\cite{krizhevsky2012imagenet, simonyan2014very, szegedy2015going, he2016deep, huang2017densely, cao2019gcnet, li2018recurrent, li2018unified, pan2016learning, qiu2017learning, simonyan2014two} have gained remarkable success on image object detection~\cite{girshick2014rich,ren2015faster,law2018cornernet,zhou2019objects,liu2016ssd,fu2017dssd}. Video object detection~(VID) extends the idea of localizing and recognizing objects in videos.  
% Sharing the same spirit with image object detection, video object detection~(VID) aims at localizing and recognizing objects in videos, 
But beyond single image, video object detection is a more challenge task which suffers from difficulties like motion blur, out-of-focus and occlusion.
% suffers from difficulties like motion blur, out-of-focus and occlusion. 

% \zhangh{In fact, videos contain various temporal cues which can be exploited to address those problems. 
% As videos exhibit \geng{temporal continuity}, the detection information from \geng{neighboring frames} can be used to refine the predictions of current frame. }
% \geng{In fact, videos contain various temporal cues from salient views of objects.
% As such, the video object detection can benefit from additionally exploiting the spatio-temporal correlations in the sequence.}

%\begin{figure}[bpt]
%    \centering
%    \includegraphics[width=\linewidth]{img/analysis2.pdf}
%    \caption{\textbf{Visualize and analyze the results from SELSA.} We provide the precision and recall, AP in the (a), (b) respectively. To futher reveal the contribution of bounding boxes with different confidence to AP/TP, we statistically accumulate $\Delta$AP/$\Delta$TP over confidence scores and overlaps with groundtruth in bins, as shown in the (d)/(e). 
%    Meanwhile, the misalignment between confidence scores and overlaps is shown in the scatter plot (c), which demonstrates  the network lacks the ability to recognize proposals accurately.
    %a) the precision/recall curve;b) the AP curve; c) The influence of overlap~(ov) and confidence~(conf) one AP increment~(deltaAP); d) The influence of overlap and confidence one TP increment~(deltaTP); e) The scatter plot of confidence vs. overlap.
%    }
%    \label{fig:analysis2}
%\end{figure}

% Currently, the accuracy of existing VID algorithms are mostly evaluated with Average Precision~(AP) or mean Average Precision~(mAP) where the predictions are selected based on the confident scores. However, such evaluation metric ignores the relations of bounding box overlap with groundtruth and the prediction scores. Fig.~\ref{fig:analysis2} show illustrates the relations of AP, True Positive~(TP) over the corresponding variables. 
%the mAP is boosted from $80.07\%$ to $93.66\%$, which is the maximum of recall. 
%To investigate the relation between localization and recognition in video streams, we reproduce the results of SELSA~\cite{wu2019sequence}, which is the previous state-of-the-art method. 
%Fig.~\ref{fig:analysis2} visualizes the result of \textit{bus} category to illustrate the relations of Average Precision~(AP), True Positive~(TP) over the corresponding variables. Based on the empirical evaluation, we make two observations. First, although predictions with high confidence scores play as central roles in AP and TP in Fig.~\ref{fig:analysis2}(a, b). Nevertheless, there still left a set of correct predictions who are with low confidence in Fig.~\ref{fig:analysis2}(d, e). Second, through Fig.~\ref{fig:analysis2}(d, e), we can find that there is a highly correlation between the confidence score and bounding box overlap from the statistical perspective. But in fact, high confidence scores do not correspond to high overlap, as shown in Fig.~\ref{fig:analysis2}(c). Moreover, to further explore the relation of overlap and confidence scores, we slightly modify the widely used evaluation metric mean Average Precision~(mAP). Specifically, we sort the detection predictions based on the overlaps with groundtruth instead of the confidence scores. As shown in Fig.~\ref{fig:analysis2}(b), there is a gap between AP $80.07\%$ and the maximum value $93.66\%$, which is bounded by the recall. It demonstrates that the network is able to localize almost of the objects but lack the ability to recognize them accurately.
%\zhangh{show what...}
%the AP $80.07\%$ can be boosted to $93.66\%$, which is its maximum value bounded by the recall. 
% \geng{
% In Fig.~\ref{fig:analysis2}, the result of \textit{bus} category is used to illustrate the relations of Average Precision~(AP), True Positive~(TP) over the corresponding variables. 
% Comparing Fig.~\ref{fig:analysis2}(a) and (b), AP is mainly determined by the bounding box with high confidence. As the analysis about the contributions to AP/TP of bounding box with different confidence and overlap in Fig.~\ref{fig:analysis2}(d) and (e), the confidence and the bounding box overlap have a highly positive correlation from the statistical perspective. However, it should be noted that there still left a set of correct predictions who are with low confidence, or vise versa.
% As shown in Fig.~\ref{fig:analysis2}(c), the confidence can not be used as a strong indicator, which leads to the gap between AP $80.07\%$ and the maximum value bounded by the recall $93.66\%$.
% It demonstrates that the network localizes almost of the objects but lacks the ability to recognize them.
% }


% To further understand the attention mechanism, we quantitatively analyze the relations of Average Precision~(AP), True Positive~(TP) over the corresponding variables in Fig.~\ref{fig:analysis2}. Based on the empirical evaluation, we make two observations. First, from Fig.~\ref{fig:analysis2}(c), the confident score and the bounding box overlap have a highly positive correlation from the statistical perspective. But in fact, high confident scores do not correspond to high overlap, or vise versa.\zhangh{which figure} Second, although predictions with high confident scores play as central roles to improve AP and TP. However, there still left a set of correct predictions with low confident in Fig.~\ref{fig:analysis2}(e).

% The advances in Convolutional Neural Networks~(CNN) have successfully improved the state-of-the-art technologies of image and video understanding~\cite{krizhevsky2012imagenet, simonyan2014very, szegedy2015going, he2016deep, huang2017densely, cao2019gcnet, li2018recurrent, li2018unified, pan2016learning, qiu2017learning, simonyan2014two}. 
% Beyond image object detection, video object detection~(VID) is a more challenge task which 
% suffers from difficulties such as fast motion, camera defocus and occlusion. Rich spatio-temporal contexts can be aggregated into single visual cues to mitigate them.

% \paragraph{Image object detection.} As one of the most fundamental tasks, object detection has been boosted since the work of R-CNN~\cite{girshick2014rich}. Instead of Selective Search~\cite{uijlings2013selective}, Faster RCNN~\cite{ren2015faster} utilized anchor mechanism to achieve great performance promotion as well as faster speed in an end-to-end manner. This kind of two-stage detector pipeline is one of the main paradigms. Furthermore, the anchor-free method~\cite{law2018cornernet,zhou2019objects} and one-stage methods~\cite{liu2016ssd,fu2017dssd} more or less borrow the ideas of the above work.
Several studies have been carried out to utilize the temporal cues to align the performance of localizing and recognizing objects in videos. Box-level association methods~\cite{feichtenhofer2017detect,han2016seq,kang2016object,kang2017object,kang2017t} link bounding boxes of each frame according to different constraints. Spatio-temporal feature aggregations~\cite{wang2018fully,xiao2018video,zhu2018towards,zhu2017flow,wu2019sequence,deng2019relation,chen2020memory} augment features by capturing contexts across adjacent frames. 
More recent works~\cite{wu2019sequence,deng2019relation,chen2020memory} have shown that attention-based operators can generate more powerful aggregation features to obtain more accurate and stable predictions. As an object appears at different `snapshots' in a video, the attention operators are capable of reducing the features variance via extracting highly semantically similar pair-wise contexts. Unfortunately, such pair-wise aggregations are usually unsatisfactory in the dissimilar features, which are hard to associate with salient views.
%\geng{Thus the pair-wise aggregations are usually unsatisfactory in the hard cases when dissimilar features can not associate with salient views.} 
For example, 
%Fig.~\ref{fig:analysis} illustrates the detection results of \emph{bus} category\geng{
several frames containing the \emph{bus} category are visulized in Fig.~\ref{fig:analysis}, which are the results of attention-based SELSA~\cite{wu2019sequence}. One can observe that after passing the context information from adjacent proposals, the recognition ability of \emph{bus} is increasing. However, as shown in Fig.~\ref{fig:analysis}($I_1$), there is limited improvement when the appearance of object vary substantially. Moreover, the prediction of the salient object will be interfered by other proposals~(\emph{bus} is wrongly categorized as \emph{car} after the propagation in Fig.~\ref{fig:analysis}($I_3$))

% the aggregation features can be more powerful if the variance of features are reduced. Attention-based operators~\cite{wu2019sequence,deng2019relation,chen2020memory} are proposed to extract highly correlated pair-wise contexts, which allow the great quantity of information available in neighboring frames help obtain more accurate and stable object detection in videos.
% \paragraph{Video Object detection.} There are mainly two directions to localize and recognize objects in videos. \textbf{a)} Box-level spatio-temporal association~\cite{feichtenhofer2017detect,han2016seq,kang2016object,kang2017object,kang2017t} match bounding boxes from frames according to different constraints. \textbf{b)} Spatio-temporal feature aggregation~\cite{wang2018fully,xiao2018video,zhu2018towards,zhu2017flow,wu2019sequence,deng2019relation,chen2020memory} augment features by aggregating related contexts from adjacent frames in time and space.

% Since the attention-based operators are introduced, pair-wise feature aggregation methods~\cite{wu2019sequence,deng2019relation,chen2020memory} characterize the relations between objects to boost performance. In the literature, there has been strong evidences on the use of object relation to support video object detection.

% \paragraph{Going deep into attention mechanism in VID.} To analyze the attention mechanism both qualitatively and quantitatively, we reproduce the results of SELSA~\cite{wu2019sequence}, which imports attention module to aggregate features in the full sequential level. 

\begin{figure}[bpt]
    \centering
    \includegraphics[width=\linewidth]{img/analysis.pdf}
    \caption{\textbf{Example output of frames containing \textit{bus} categroy}. The first row is the result without temporal aggregation, which is produced by the single frame version of SELSA, and the second row is the result which aggregates pair-wise context from support frames. 
    }
    \label{fig:analysis}
\end{figure}

% As shown in Fig.~\ref{fig:analysis}, we visualize the result of \textit{bus} category to analyze the problems in it. 
% In Fig.~\ref{fig:analysis}(a,b), the recognition ability of buses is improved with the context from other proposals.
%the network combined the context from other proposals to improve the recognition ability.
% Unfortunately, the proposals with quite different appearance from others has limited improvements with the attention mechanism. However, they are often hard cases in the detection process. Furthermore, discriminative discriminative enough may be confused by other proposals.

%Through the visualization on Fig~\ref{fig:analysis2}(a-e),

% among main indicator AP, TP, confidence with their dependent variables.
% Here, two problems in the result are revealed as follows: a) Although there is a statistically positive correlation between confidence and overlap, it can be found that confidence cannot be used as an indicator of overlap; b) The predictions with high confidence indeed make the biggest contribution to AP and TP. However, there still left some correct predictions with low confidence. 

%To explore the attention-based mechanism more deeply, we firstly slightly modify the common metric Mean Average Precision~(mAP). Specifically, we sort the detection results according to the overlap with groundtruth, instead of origin objectness scores. The same prediction result is boosted from $80.07\%$ to $93.66\%$. It shows that this result has covered most of the objects to be detected in the video. Furthermore, we visualize the result of \textit{bus} category in Fig.~\ref{fig:analysis}~(c-g) and analyze the problems in it. 
%Through this visualization, several problems in the result are revealed as follows:

%1) The predictions with high confidence indeed make the biggest contribution to AP. However, there still left some correct predictions with low confidence;

%2) With decreasing of confidence, the proportion of correct prediction is reducing;

%3) Although there is a statistically positive correlation between confidence and overlap, it can be found on Fig~\ref{fig:analysis}(e) that confidence cannot be used as an indicator of overlap.

%It can be seen that improving the recognizing power of the network has a greater effect on video object detection than the localization accuracy of bounding boxes. As a video-level object-aware prior, knowing what is there in the video can simplify video object detection to finding it in the frames. 
%It can be realized by aggregating more global context about objects in the video.

%\zhangh{As a video-level object-aware prior, knowing what is there in the video can simplify video object detection to find it in the frames.}
% With the video-level object aware prior, video object detection is reinterpreted from a sequential detection task to a query of specific object in frames.
By consolidating the idea of modeling spatial-temporal context, in this paper, we propose \modulename{}~(\modulenameshort{}) module for video object detection. The \modulenameshort{} module extracts the video-level object-aware knowledge, and highly boosts the performance via augmenting such prior knowledge with the well-established pair-wise contexts.
Our approach is motivated by the intriguing observation that when people are not certain about the identity of an object with a deteriorated appearance in the current frame, it is natural to seek the existence of objects in the video and assign them with the most similar objects.
Therefore, by borrowing this idea from human,  we simplify the video object detection as querying specific object in frames.

Specifically, our \modulenameshort{} module augments features from proposals generated by Region Proposal Network~(RPN). We split the input features into two parts and feed into separate paths, \ie, \textit{semantic path} and \textit{localization path}, to aggregate classification and localization features independently.
In the semantic path, we first collect the object-aware knowledge from proposals across the whole video. Meanwhile, the semantic context is obtained via calculating the pair-wise similarity among reference frames. By aggregating above pair-wise semantic context and object-aware knowledge of proposals, the features encode more knowledge about other regions and the whole video.
% semantic features from reference frames firstly aggregate other features by pair-wise similarities. Meanwhile, we collect the object-aware knowledge of proposals in all the sequence, especially which correspond to regions containing the whole or part of objects. Aggregating above pair-wise semantic context and object-aware knowledge of proposals, the features encode more knowledge about other regions and the whole video. 
In the localization path, localization features are also augmented with pair-wise localization context. In contrast to the semantic path, we locally enhance the features which ensures the features to be sensitive to relative postions.
% However, to ensure the features to be sensitive to relative position, we augment features locally.
%  maintain sensitive to the relative position, we only augment the localization features without global context.
To futher improve the performance, we design a post-processing algorithm named Sequence DIoU NMS. Instead of linking the bounding boxes according to intersection of union~(IoU), we perform Distance-IoU~(DIoU)~\cite{zheng2020distance} to associate and supress boxes in videos. 

Though being simple, the proposed \modulenameshort{} module achieves surprisingly good performance, and it is able to complement existing attention-based video object detection methods. Extensive empirical evaluations explicitly demonstrate that the proposed method is competitive in performance. Furthermore, we conduct ablation experiments to analyze the effects of various design choices in \modulenameshort{} module.

% Moreover, the learned \modulenameshort{} module also benefits the post-processing of Sequence DIoU NMS.
% \geng{Being consistent with similar approaches, our learned \modulenameshort{} also benefits from the post-processing method to further improve the performance, such as the Sequence DIoU NMS in this paper. Note that our \modulenameshort{} module can be introduced in other proposal-based tasks.}



%Region Proposal Network~(RPN) produces object proposals from input frames. Then our \modulenameshort{} augments splitted features of object proposals in two paths for classification and localization. 
%For classification feature aggregation, features from reference frames are measured similarities with the other semantic features. Meanwhile, we extract the object-aware knowledge of proposals, which correspond to regions containing the whole or part of objects. Aggregating pair-wise semantic context and object-aware knowledge of proposals, the features encode more knowledge about other regions and the whole video. For localization feature augmentation, features are measured similarities with other localization features to keep sensitive to the relative position. 
%, features from reference frames are measured similarities with the other semantic features. Meanwhile, we extract the object-aware knowledge of proposals, which correspond to regions containing the whole or part of objects. Aggregating pair-wise semantic context and object-aware knowledge of proposals, the features encode more knowledge about other regions and the whole video. For localization feature augmentation, features are measured similarities with other localization features to maintain sensitive to the relative position. 
%Considering the contradiction between classification and regression, we only augment the splitted loc-features to keep sensitive to the relative position. 
%Moreover, the learned \modulenameshort{} also benefits the post-processing of Sequence DIoU NMS.

% which does not strongly utilize global context of the scene.

==> intro_bk_99.tex <==
\section{Introduction}
\label{Introduction}
Convolutional neural networks~(CNNs)~\cite{krizhevsky2012imagenet, simonyan2014very, szegedy2015going, he2016deep, huang2017densely, cao2019gcnet, li2018recurrent, li2018unified, pan2016learning, qiu2017learning, simonyan2014two} have gained remarkable success in image object detection~\cite{girshick2014rich,ren2015faster,law2018cornernet,zhou2019objects,liu2016ssd,fu2017dssd}. Video object detection~(VID) extends the idea of localizing and recognizing objects in videos.  
But beyond the single image, video object detection is a more challenging task that suffers from difficulties like motion blur, out-of-focus and occlusion.

Videos contain various temporal cues which can be exploit to improve the performance of localizing and recognizing. Several studies have been carried out to exloit the spatial-temporal context in vodeo object detection.
% By consolidating the idea of modeling the spatial-temporal context, several studies have been carried out to utilize the temporal cues to improve the performance of localizing and recognizing objects in videos. 
% Box-level association methods~\cite{feichtenhofer2017detect,han2016seq,kang2016object,kang2017object,kang2017t} and feature aggregations across adjacent frames~\cite{wang2018fully,xiao2018video,zhu2018towards,zhu2017flow} accumulate context or associate detections over time.
Box-level association methods~\cite{feichtenhofer2017detect,han2016seq,kang2016object,kang2017object,kang2017t} link bounding boxes of each frame according to different constraints. 
Spatio-temporal feature aggregations~\cite{wang2018fully,xiao2018video,zhu2018towards,zhu2017flow,wu2019sequence,deng2019relation,chen2020memory} augment features by capturing contexts across adjacent frames. 
% Lifting time limitation, 
More recent works~\cite{wu2019sequence,deng2019relation,chen2020memory} have shown that attention-based operators can generate more powerful features to obtain more accurate and stable predictions. As the attention operators are capable of reducing the variance within features via extracting highly semantically similar pair-wise contexts from the whole sequence. 
% an object appears at different `snapshots' in a video, 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{img/analysis.pdf}
    \caption{
        %\textbf{Example output of frames containing \emph{bus} categroy}. The first row is the result without temporal aggregation, which is produced by the single frame version of SELSA, and the second row is the result which aggregates pair-wise context from support frames. 
        \textbf{Example output of the attention-based approach}~\cite{wu2019sequence}. The first row is the result without temporal aggregation, which is produced by the single frame version of SELSA, and the second row is the result which aggregates pair-wise context from support frames. After passing the context information from other proposals, the recognition ability of \emph{bus} is increasing. However, as shown in $I_1$, there is limited improvement when the appearance of the object varies substantially. Moreover, the prediction of the salient object will be interfered by other proposals~(\emph{bus} is wrongly categorized as \emph{car} after the propagation in $I_3$).
    }
    \label{fig:analysis}
\end{figure}

%Unfortunately, the above methods focus on short time windows or pair-wise relations, which have less idea about global video content. Such as the pair-wise aggregation, it is usually unsatisfactory in the dissimilar features, which are hard to associate with salient views. For example, several frames containing the \emph{bus} category are visualized in Fig.~\ref{fig:analysis}, which are the results of attention-based SELSA~\cite{wu2019sequence}. One can observe that after passing the context information from other proposals, the recognition ability of \emph{bus} is increasing. However, as shown in Fig.~\ref{fig:analysis}($I_1$), there is limited improvement when the appearance of the object varies substantially. Moreover, the prediction of the salient object will be interfered by other proposals~(\emph{bus} is wrongly categorized as \emph{car} after the propagation in Fig.~\ref{fig:analysis}($I_3$)). Considering the gap between AP of \emph{bus} $80.07\%$ and the maximum value $93.66\%$ bounded by the recall, it demonstrates that the network localizes almost of the objects but lacks the ability to recognize and associate them accurately, which is one of the existing bottlenecks of VID. 
Existing works modelling the spatial-temporal contexts mainly focus on short-time window or pair-wise feature relations. In comparison, less effort has been made to extract the global video content. But in fact, an object in different frames usually have quite different views, and associating such dissimilar features with the salient views can be very hard.
We reprodce the results of SELSA~\cite{wu2019sequence}, and Fig.~\ref{fig:analysis} visualized several frames containing the \emph{bus} category. 
The average precision~(AP) of \emph{bus} is $80.07\%$, however, bounded by the recall, the maximum value of AP can be achieved to $93.66\%$. The huge gap demonstrates that the network is able to localize almost of the objects but lacks the ability to recognize them accurately.
For example, as shown in Fig.~\ref{fig:analysis}, one can observe that after passing the context information from other proposals, the recognition ability of \emph{bus} is increasing. However, as shown in Fig.~\ref{fig:analysis}($I_1$), there is limited improvement when the appearance of the object varies substantially. Moreover, the prediction of the salient object will be interfered by other proposals~(\emph{bus} is wrongly categorized as \emph{car} after the propagation in Fig.~\ref{fig:analysis}($I_3$)). \zhangh{to global content}

% Unfortunately, the above methods focus on short time windows or pair-wise relations, which have less idea about global video content. Such as the pair-wise aggregation, it is usually unsatisfactory in the dissimilar features, which are hard to associate with salient views, which can be proven in the cases visulized and analyzed in Fig.~\ref{fig:analysis}. Considering the gap between AP of \emph{bus} $80.07\%$ and the maximum value $93.66\%$ bounded by the recall, it demonstrates that the network localizes almost of the objects but lacks the ability to recognize and associate them accurately, which is one of the existing bottlenecks of VID. 
%Hence, it is one of the existing bottlenecks of VID to achieves capable representation for classification and proposal association.

In this paper, we propose the \modulename{}~(\modulenameshort{}) module for video object detection. The \modulenameshort{} module extracts the video-level object-aware knowledge, and highly boosts the performance via augmenting such prior knowledge with the well-established pair-wise contexts.
Our approach is motivated by the intriguing observation that when people are not certain about the identity of an object with a deteriorated appearance in the current frame, it is natural to seek the existence of objects in the video and assign them with the most similar objects.
Therefore, by borrowing this idea from humans,  we simplify the video object detection as querying specific objects in frames.
%can be used to eliminate confusion to recognition objects 
% Our approach is motivated by the intriguing observation that when people are not certain about the identity of an object with a deteriorated appearance in the current frame, it is natural to seek the existence of objects in the video and assign them with the most similar objects. 
% Therefore, with the \emph{object-ware knowledge}, which provides object categories contained in the video, we can simplify the video object detection as querying specific objects in frames.
% In this paper, we propose the \modulename{}~(\modulenameshort{}) module for video object detection, which highly boosts the performance via augmenting object-aware knowledge with the well-established pair-wise contexts.
%The \modulenameshort{} module extracts the video-level object-aware knowledge, and highly boosts the performance via augmenting such prior knowledge with the well-established pair-wise contexts.

%Specifically, our \modulenameshort{} module augments features from proposals generated by Region Proposal Network~(RPN). 
%We split the input features into two parts and feed into separate paths, \ie, \textit{semantic path} and \textit{localization path}, to aggregate semantic and localization features independently.
Specifically, our \modulenameshort{} module augments features corresponding to proposals in all the frames.
The input features are split into two parts and fed into separate paths, \ie, \emph{semantic path} and \emph{localization path}:

a) \textbf{Semantic path.} We first collect the object-aware knowledge from proposals across the whole video. Meanwhile, the pair-wise semantic context is obtained via calculating similarity between proposals. By aggregating above pair-wise semantic context and object-aware knowledge of proposals, the features encode more knowledge about other regions and the whole video.
%Meanwhile, the semantic context is obtained via calculating the pair-wise similarity among reference frames. By aggregating above pair-wise semantic context and object-aware knowledge of proposals, the features encode more knowledge about other regions and the whole video.

b) \textbf{Localization path.} Localization features are also augmented with the pair-wise localization context. In contrast to the semantic path, we locally enhance the features to ensure the features sensitive to relative positions.

To further improve the performance, we propose an efficient post-processing strategy named Sequence DIoU NMS. Instead of linking the bounding boxes according to the intersection of union~(IoU), we perform Distance-IoU~(DIoU)~\cite{zheng2020distance} to associate and suppress boxes in videos. 

Though being simple, the \modulenameshort{} module achieves surprisingly good performance, and it is easy to complement existing attention-based and proposal-based video object detection methods. Extensive empirical evaluations explicitly demonstrate that the proposed method is competitive in performance. Furthermore, we conduct ablation experiments to analyze the effects of various design choices in the \modulenameshort{} module.


==> method_bk_827.tex <==
\section{Method}
\label{method}

In this section, we first set up the two-stage object detection pipeline. Then we discuss our proposed xxx to improve the training in detail. Roughly, xxx. yyy xxx.

% We refer to the new CNN module as \textit{\modulename{}} and the components of the module are illustrated in Fig.~\ref{fig:overview}. We devise this module to facilitate video object detection by augmenting features in parallel and different aggregation paths.

% \subsection{Two-stage Object Detection}

% To be specific, we take the most typical method: Faster RCNN~\cite{ren2015faster} as an example to introduce details of such framework, whose settings are widely used by followers. When new image comes, dense feature representations are extracted by a pretrained convolutional neural network. The next step is to produce object proposals by Region Proposal Network~(RPN), which simultaneously predicts object bounds and objectness scores. Usually, the RoI operators, \ie RoI-pooling, RoI-align in Faster RCNN extracts a fixed-length feature vector from the feature map, which is exploited for subsequent proposal classification and regression.

% Revisiting faster-rcnn-style detection pipelines, a pretrained CNN extract dense convolutional featuremaps. Then the Region Proposal Network~{(RPN)} produces object proposals, which contain object scores and proposal coordinates. Usually, RoI operaters~(\ie, RoI-pooling, RoI-align) are exploited to extract object features from the predicted proposal regions, which is exploited for subsequent proposal classification and regression.


%feed the trunked the $f_{obj}$ into $f_{cls}$ and $f_{loc}$ into our Cls-Loc Aggregation Module, in which these two features are upgraded individually.
%trunk the $f_{obj}$ into $f_{cls}$ and $f_{loc}$.
%the object scores $s_{obj}$ of proposals are the predicted probability of given anchors being objects. 

%Given input reference frame $I_{t}$ and support frames $I_{t-T}$ and $I_{t+T}$, we first use a pre-trained CNN to extract dense convolutional featuremaps. Then the Region Proposal Network~{(RPN)} produces object proposals from reference frame and all support frames, which contain object scores $s_{obj}$ and proposal coordinates. Usually, RoI operaters~(\ie, RoI-pooling, RoI-align) are exploited to extract object features $f_{obj}$ from the predicted proposal regions, which is exploited for subsequent proposal classification and regression.
%However, there is several contradiction between classification and regression. Proposal classification is designed to be insensitive to position, which means different $f_{obj}$ from the same object should produce same classification results. In contrast, proposal regression is designed to be sensitive to relative position. This puts contradictory requirements on $f_{obj}$.

%We decouple the faster-rcnn-style network, and further carry out similar but different designs for the classification and regression tasks.
%Here, we feed the trunked the $f_{obj}$ into $f_{cls}$ and $f_{loc}$ into our Cls-Loc Aggregation Module, in which these two features are upgraded individually.

%trunk the $f_{obj}$ into $f_{cls}$ and $f_{loc}$.
%the object scores $s_{obj}$ of proposals are the predicted probability of given anchors being objects. 

\subsection{Overview}
\zhangh{Given frames sampled from the same video, we use the share-weight backbone to predict proposals and extract corresponding features. In our \modulenameshort{}, the features from the reference frame are updated. According to the different supervision signals, our \modulenameshort{} are splitted into classification branch and localization branch. In the classification branch, the input features, $f^{cls}$, aggregate the classification context of the proposals and the global context of all proposals. In the localization branch, the input features, $f^{loc}$, are augmented for subsequent localization.  With different supervision signals and learnable context aggregation operators, parallel branches can alleviate the contradiction between two tasks. Stacking \modulenameshort{}s multiple times, the augmented features are separately used for classification and localization.}
% \hspace{0.5cm} 
\paragraph{Two-stage Object Detection.}
We take the most typical method: Faster RCNN~\cite{ren2015faster} as an example to introduce details of such framework, whose settings are widely used by followers. When new image comes, dense feature representations are extracted by a pretrained convolutional neural network. The next step is to produce object proposals by Region Proposal Network~(RPN), which simultaneously predicts object bounds and objectness scores. Usually, the RoI operator, \eg RoI-pooling, RoI-align, in Faster RCNN extracts a fixed-length feature vector from the feature map, which is exploited for subsequent proposal classification and regression. However, due to the goal of classification is contradict to regression, the shared features produced by RoI operator are difficult to trade classification for regression, or vise versa. As bounding box regression aims at localizing objects, which is position-sensitive, while classification is to distinguish different objects.

% Usually, the RoI operators, \ie RoI-pooling, RoI-align in Faster RCNN extracts a fixed-length feature vector from the feature map, which is exploited for subsequent proposal classification and regression.

% However, there is several contradiction between classification and regression. Proposal classification is designed to be insensitive to position, which means features corresponding to the same object should produce same classification results. In contrast, proposal regression is designed to be sensitive to relative position. This puts contradictory requirements on feature extraction and augmentation.

% We decouple the faster-rcnn-style network, and further carry out similar but different designs for the classification and regression tasks.
% Here, our \textit{\modulename{}} contains two parallel paths, in which cls-features and loc-features are upgraded individually. 

\paragraph{Revisiting SOTA VID Method.} \zhangh{SELSA imported attention-based operators to aggregate features in the full-sequence level. With repeated aggregation, features are more discriminative and robust. It has a great impact on subsequent RDN and MEGA.} We reproduce the results from SELSA~\cite{wu2019sequence}, which are one of the state-of-the-art methods, to analysis the possible improvements. We firstly slightly modify the common metric Mean Average Precision~(mAP). Specifically, we sort the detection results according to the overlap with groundtruth, instead of origin objectness scores. The same prediction result is boosted from $57.01\%$ to $69.06\%$. It shows that this result has covered most of the objects to be detected in the video. Furthermore, we visualize the result of monkey category in Fig.~\ref{fig:analysis} and analyze the problems in it. In this visualization, several problems in the result are revealed, as follows:

1) The predictions with high confidence did make the biggest contribution to AP. However, there were also some correct predictions with low confidence;

2) With the decrease of confidence, the proportion of correct prediction is decreasing;

3) Although there is a statistically positive correlation between confidence and overlap, it can be found on the scatter plot that confidence cannot be used as an indicator of overlap.

It can be seen that to improve the recognizing power of network has a greater effect on video object detection than to improve the localization accuracy of bounding boxes. It can be realized by aggregating more global context about objects in the video.

\begin{figure}[bpt]
    \centering
    \includegraphics[width=\linewidth]{img/analysis.pdf}
    \caption{\textbf{Visualize and analyze the results from SELSA}.a) the precision curve; b) the recall curve;c) the AP curve~(red) and the prediction indexes; d) The influence of overlap~(ov) and confidence~(conf) one AP increment~(deltaAP); e) The influence of overlap and confidence one TP increment~(deltaTP); f) The scatter plot of confidence vs. overlap.
    }
    \label{fig:analysis}
\end{figure}

\subsection{Two-path Feature Aggregation Module}
Video object detection aims at recognizing and localizing objects for each frame of video ${\{I_t\}_{t=1}^T}$. 

\subsection{Our method}

\paragraph{\textit{Notation.}} At first, we define some notations which will be used in following. The goal of video object detection is to recognize and localize objects for every frame of video ${\{I_t\}_{t=1}^T}$, where the index sequence ${\{1,...,T\}}$ is the time stamps of input frames.
With pretrained CNN backbone, feature maps ${\{M_t\}_{t=1}^T}$ are extracted.
Given the current frame $I_t$, RPN generate proposals ${B_t=\{b_t^i\}}$ and corresponding objectness scores $S_t=\{s_t^i\}$ at each frame. Furthermore, we represent proposal features $f^{obj}_{t,i}$ extracting from ${b_t^i}$.

\paragraph{Context Aggregation.} To mine the relationship between proposals from each frame, the attention-based operators~\cite{vaswani2017attention, wu2019sequence} are employed. Let $F^*=\{f^*_i\}$ denote the features from all frames, a general attention-based operator enhances features via reweighting features from other proposals with learnable parameters. The ${F^{agg} = \{f^{agg}_i\}}$ can be computed as
% a learnable weighted sum of features from other proposals. 
% Given proposals ${B=\{b_i\}}$, objectness scores ${S=\{s_i\}}$ and features ${F^*=\{f^*_i\}}$ from all the frames, a general attention-based operator enhance features by a learnable weighted sum of features from other proposals. The ${F^{agg} = \{f^{agg}_i\}}$ can be computed as

\begin{equation}
    \begin{aligned}
        Q(F^*) &= W^*_q \cdot F^*, \\
        K(F^*) &= W^*_k \cdot F^*, \\
        Att(f^*_i, F^*) &= softmax(\frac{Q(f^*_i)K(F^*)^T}{\sqrt d}) F^*, \\
        f^{agg, *}_i &= f^*_i + Att(f^*_i, F^*).
    \end{aligned}
\end{equation}


where both $W^*_q$ and $W^*_k$ are linear learnable transformation matrices. $d^*$ is the dimension of $F^*$.

\subsubsection{Two-path Feature Aggregation Module}\
\newline
\indent In our \modulenameshort{}, we devide $f^{obj}_i$ into $f^{cls}_i$ and $f^{loc}_i$. Here, we optimize those two features via feeding those two features into the following two independent paths.

\textbf{Path1: Cls-Context Aggregation and Global Feature of Proposals.}
The occluded or blurred objects in current frames may appear clearly in the neighbouring frames. And other objects in the scene can also help recognize the proposals. Hence, we firstly employ a Cls-Context Aggregation operator to augment features. Through operator simply captures the relationship between different proposals, however it lacks the ability acquire the global context of the entire video. Hence, we devote to study to extract and aggregate global context of the video.

\textbf{Global context of frames.} Inspired by global context extraction in semantic segmentation~\cite{liu2015parsenet, zhao2017pyramid}, the global context of frames can be computed as

\begin{equation}
    \begin{aligned}
        G_{gcf}(\{M_t\}_{t=1}^T) &= Mean(\{M_t\}_{t=1}^T).
    \end{aligned}
    \label{eq:gcf}
\end{equation}

However, most of frames are with messy background, and objects only occupy a small region. Consequently, the extracted global context features contain limited knowledge about the objects.

% objects only occupy a small part the objects only occupy a small part of the entire video, and most of it is a messy background. As a result, the extracted global context only contains a small amount of global context about the objects in the frames.

\textbf{Global context of proposals.}
In the test phase of faster-rcnn-style network, proposals mainly focus on the part of the scene where objects may exist and most of the background is filtered out. Therefore, feature extraction at proposal-level can better know the global context of objects in the video, which can be computed as
\begin{equation}
    G_{gcp}(F^{cls}) = Mean(F^{cls}).
    \label{eq:gcp}
\end{equation}
However, the proposals also contains some false negative cases. Even though these proposals include a part of the object, these information can not help to extract accurate global context due to bias. 

\textbf{Highlight features from proposals within objects.}
To further expand the idea of extracting the global context of proposals, our approach is designed to emphasize high-quality proposal. Through observation, we find that proposals with high objectness scores produced by RPN mostly contains the main body or salient parts of the objects. And a large number of proposals can eliminate the uncertainty of the objectness scores for proposal quality evaluation. Specifically, we introduce the objectness score to weight different features corresponding to proposal, and in order to ensure the stability of the feature, we further normalize it, as follows:
\begin{equation}
    G_{hgcp}(F^{cls}) = \frac{\sum_i(s_i \times f^{cls}_i)}{\sum_i(s_i)}.
    \label{eq:hgcp}
\end{equation}
In order to synthesize Cls-Context aggregation and global feature of proposals, we calculate a set of factors from the output from equation~\ref{eq:hgcp} to selectively hightlight the class-dependet channels of aggregated features, as equation~\ref{eq:cls},
\begin{equation}
    f^{Video} = Softmax(NL(G_{hgcp}(F^{cls})))\cdot F^{agg,cls},
    \label{eq:cls}
\end{equation}
where $NL(\cdot)$ is non-linear transformations applied to the global context of proposals.

\textbf{Path2: Loc-Context Aggregation.} As previous analysis, the existing networks are employable to localize objects. However, to avoid the interference of too many contexts, we still adopt an independent Loc-Context Aggregation operator. The augmented $F^{agg,loc}$ can be trained only under the supervision of the annotated coordinates of bounding boxes.

\subsubsection{Sequence DIoU NMS}
\
\newline
\indent\textbf{Sequence NMS.} Seq-NMS~\cite{han2016seq} is a classical post-processing for sequence detection. However,  
for objects that are dense and occlude each other in consecutive frames, Seq-NMS links the bounding boxes according to overlaps that will cause two different objects to be processed in a tubelet.

\textbf{Action Tube and BLR.} Different from the thresholded linking criterion in ~\cite{han2016seq}, action tube~\cite{gkioxari2015finding} added overlaps into the optimization goal, which made the selecte sequence more smooth in space and had more opportunity to link the same objects in different frames. BLR~\cite{deng2019relation} further added the pair-wise relation weight from network into the optimization goal to process and optimize multiple frames at the same time, which also limited its application due to the necessary relation output.

\textbf{DIoU NMS.} In fact, in image object detection, the false non-maximum suppression is also a problem still to be solved. DIoU NMS~\cite{zheng2020distance} is an extended overlap metric. Different from jaccard overlap, DIoU NMS considered the center distance of bounding boxes, which has better effect to distinguish crowded objects.

\textbf{Our approach.} Note that since sequence selection is a key and difficult point in processing bounding boxes in frames, we improve the Seq-NMS with DIoU. Our post-processing operator can improve the performance significantly while maintaining the flexibility of origin methods, as shown in algrithms~\ref{alg:seq-dnms}.

\begin{algorithm}[htb] 
    \SetAlgoNoLine
    \caption{Sequence DIoU-based NMS.} 
    \label{alg:seq-dnms} 
    \begin{algorithmic}[1] 
    \Require
    ${B_t=\{b_t^i\}}$,
    ${S_t=\{s_t^i\}}$,
    $\tau_1$, $\tau_2$
    \Statex$t \in \{1,...,T\}$ is the time stamp
    \Statex${B_t}$ is the list of initial bounding boxes in frame $t$
    \Statex${S_t}$ contains corresponding detection scores
    \Statex$\tau_1$ and $\tau_2$ are the threshold
    
    \Ensure optimal ${B_t=\{b_t^i\}}$, ${S_t=\{s_t^i\}}$
    \State Create linkes $L$:
    \Statex
    \For{$t=1;t \le T-1$}
    {
        $L_t = \Phi$
        \For{$b_i \in B_t and b_j \in B_{t+1}$}
        {
            \If{$DIoU(b_i, b_j)\le \tau 1$}
            {
                $L_t \cup link(b_i,b_j)$
            }
        }
        $L \cup L_t$
    }
    \State Find maximum paths:
    \Statex
    find the maximum path $P = \{b_{t_0},...,b_{t_1}\}$from $t_0$ to $t_1$,
    \While{$P \neq \Phi$ or $\sum\{s_{t_0},...,s_{t_1}\}$ or $L \neq \Phi$}
    {
        \For{$t=t_0;j \le t_1;$}
        {
            \For{$b_i \in B_t$}
            {
                \If{$DIoU(b_i, b_t)\le \tau_2$}
                {
                    delete $b_i$ and corresonding links;
                }
            }
        }
        update $L$
    }
    rescore the corresonding $\{s_{t_0},...,s_{t_1}\}$
    %\Return new ${B_t=\{b_t^i\}}$, ${S_t=\{s_t^i\}}$
    \end{algorithmic} 
    \end{algorithm}

\subsubsection{Relation to Other Approaches}
\
\newline
\indent\textbf{Multi-head attention-based approaches.} In attention-based approaches~\cite{vaswani2017attention,deng2019relation}, the multi-head attention is used to make the attention operators to model different relations to enhance each proposals. In multi-head attention, the input features are splitted into different parts, which are calculated attention weight separately. Then the all of parts are enhanced correspondingly. 
Our approach differs significantly from these in operators and motivation. Although we also split the $f^{obj}$ into two part, we use different supervision for each part, which reduce the contradiction between recognition and localization. And it needs to be emphasized that this split operator is a necessary pre-operation to extract global context of proposals.

\textbf{Global Features Aggregation.} Global context has been proven effective in semantic segmentation~\cite{liu2015parsenet,zhao2017pyramid}, action recognition~\cite{wang2018videos} and similar tasks.
In semantic segmentation~\cite{liu2015parsenet,zhao2017pyramid,zhang2018context}, both foreground and background are densely encoded into the global context, without paying more attention to foreground objects.
action recognition~\cite{wang2018videos} can obviously benefit from the global context of the video. However, for the meaningless proposals produced by detectors, no processing methods have been proposed.
To the date of submission, we are the first to adopt and improve similar strategies to extract global context in video object detection. For the redundant and overlapping proposals in object detection pipeline, we disign a weighted aggregation strategy to obtain global context of proposal. Our approach can be trained in an end-to-end manner and adapted to most two-stage detectors.

==> method_bk_827_2.tex <==
\section{Method}
\label{method}

In this section, we first set up the two-stage object detection pipeline. Then we discuss our proposed xxx to improve the training in detail. Roughly, xxx. yyy xxx.

% We refer to the new CNN module as \textit{\modulename{}} and the components of the module are illustrated in Fig.~\ref{fig:overview}. We devise this module to facilitate video object detection by augmenting features in parallel and different aggregation paths.

% \subsection{Two-stage Object Detection}

% To be specific, we take the most typical method: Faster RCNN~\cite{ren2015faster} as an example to introduce details of such framework, whose settings are widely used by followers. When new image comes, dense feature representations are extracted by a pretrained convolutional neural network. The next step is to produce object proposals by Region Proposal Network~(RPN), which simultaneously predicts object bounds and objectness scores. Usually, the RoI operators, \ie RoI-pooling, RoI-align in Faster RCNN extracts a fixed-length feature vector from the feature map, which is exploited for subsequent proposal classification and regression.

% Revisiting faster-rcnn-style detection pipelines, a pretrained CNN extract dense convolutional featuremaps. Then the Region Proposal Network~{(RPN)} produces object proposals, which contain object scores and proposal coordinates. Usually, RoI operaters~(\ie, RoI-pooling, RoI-align) are exploited to extract object features from the predicted proposal regions, which is exploited for subsequent proposal classification and regression.


%feed the trunked the $f_{obj}$ into $f_{cls}$ and $f_{loc}$ into our Cls-Loc Aggregation Module, in which these two features are upgraded individually.
%trunk the $f_{obj}$ into $f_{cls}$ and $f_{loc}$.
%the object scores $s_{obj}$ of proposals are the predicted probability of given anchors being objects. 

%Given input reference frame $I_{t}$ and support frames $I_{t-T}$ and $I_{t+T}$, we first use a pre-trained CNN to extract dense convolutional featuremaps. Then the Region Proposal Network~{(RPN)} produces object proposals from reference frame and all support frames, which contain object scores $s_{obj}$ and proposal coordinates. Usually, RoI operaters~(\ie, RoI-pooling, RoI-align) are exploited to extract object features $f_{obj}$ from the predicted proposal regions, which is exploited for subsequent proposal classification and regression.
%However, there is several contradiction between classification and regression. Proposal classification is designed to be insensitive to position, which means different $f_{obj}$ from the same object should produce same classification results. In contrast, proposal regression is designed to be sensitive to relative position. This puts contradictory requirements on $f_{obj}$.

%We decouple the faster-rcnn-style network, and further carry out similar but different designs for the classification and regression tasks.
%Here, we feed the trunked the $f_{obj}$ into $f_{cls}$ and $f_{loc}$ into our Cls-Loc Aggregation Module, in which these two features are upgraded individually.

%trunk the $f_{obj}$ into $f_{cls}$ and $f_{loc}$.
%the object scores $s_{obj}$ of proposals are the predicted probability of given anchors being objects. 

\subsection{Overview}
\zhangh{Given frames sampled from the same video, we use the share-weight backbone to predict proposals and extract corresponding features. In our \modulenameshort{}, the features from the reference frame are updated. According to the different supervision signals, our \modulenameshort{} are splitted into classification branch and localization branch. In the classification branch, the input features, $f^{cls}$, aggregate the classification context of the proposals and the global context of all proposals. In the localization branch, the input features, $f^{loc}$, are augmented for subsequent localization.  With different supervision signals and learnable context aggregation operators, parallel branches can alleviate the contradiction between two tasks. Stacking \modulenameshort{}s multiple times, the augmented features are separately used for classification and localization.}
% \hspace{0.5cm} 
\paragraph{Two-stage Object Detection.}
We take the most typical method: Faster RCNN~\cite{ren2015faster} as an example to introduce details of such framework, whose settings are widely used by followers. When new image comes, dense feature representations are extracted by a pretrained convolutional neural network. The next step is to produce object proposals by Region Proposal Network~(RPN), which simultaneously predicts object bounds and objectness scores. Usually, the RoI operator, \eg RoI-pooling, RoI-align, in Faster RCNN extracts a fixed-length feature vector from the feature map, which is exploited for subsequent proposal classification and regression. However, due to the goal of classification is contradict to regression, the shared features produced by RoI operator are difficult to trade classification for regression, or vise versa. As bounding box regression aims at localizing objects, which is position-sensitive, while classification is to distinguish different objects.

% Usually, the RoI operators, \ie RoI-pooling, RoI-align in Faster RCNN extracts a fixed-length feature vector from the feature map, which is exploited for subsequent proposal classification and regression.

% However, there is several contradiction between classification and regression. Proposal classification is designed to be insensitive to position, which means features corresponding to the same object should produce same classification results. In contrast, proposal regression is designed to be sensitive to relative position. This puts contradictory requirements on feature extraction and augmentation.

% We decouple the faster-rcnn-style network, and further carry out similar but different designs for the classification and regression tasks.
% Here, our \textit{\modulename{}} contains two parallel paths, in which cls-features and loc-features are upgraded individually. 

\paragraph{Revisiting SOTA VID Method.} \zhangh{SELSA imported attention-based operators to aggregate features in the full-sequence level. With repeated aggregation, features are more discriminative and robust. It has a great impact on subsequent RDN and MEGA.} We reproduce the results from SELSA~\cite{wu2019sequence}, which are one of the state-of-the-art methods, to analysis the possible improvements. We firstly slightly modify the common metric Mean Average Precision~(mAP). Specifically, we sort the detection results according to the overlap with groundtruth, instead of origin objectness scores. The same prediction result is boosted from $57.01\%$ to $69.06\%$. It shows that this result has covered most of the objects to be detected in the video. Furthermore, we visualize the result of monkey category in Fig.~\ref{fig:analysis} and analyze the problems in it. In this visualization, several problems in the result are revealed, as follows:

1) The predictions with high confidence did make the biggest contribution to AP. However, there were also some correct predictions with low confidence;

2) With the decrease of confidence, the proportion of correct prediction is decreasing;

3) Although there is a statistically positive correlation between confidence and overlap, it can be found on the scatter plot that confidence cannot be used as an indicator of overlap.

It can be seen that to improve the recognizing power of network has a greater effect on video object detection than to improve the localization accuracy of bounding boxes. It can be realized by aggregating more global context about objects in the video.

\begin{figure}[bpt]
    \centering
    \includegraphics[width=\linewidth]{img/analysis.pdf}
    \caption{\textbf{Visualize and analyze the results from SELSA}.a) the precision curve; b) the recall curve;c) the AP curve~(red) and the prediction indexes; d) The influence of overlap~(ov) and confidence~(conf) one AP increment~(deltaAP); e) The influence of overlap and confidence one TP increment~(deltaTP); f) The scatter plot of confidence vs. overlap.
    }
    \label{fig:analysis}
\end{figure}

\subsection{Two-path Feature Aggregation Module}
\paragraph{\textit{VID notation.}} At first, we define some notations which will be used in the following. Video object detection aims at recognizing and localizing objects for each frame of video ${\{I_t\}_{t=1}^T}$, where the index sequence ${\{1,..., T\}}$ is timestamps of input frames.
With pretrained CNN backbone, feature maps ${\{M_t\}_{t=1}^T}$ are extracted.
Given the current frame $I_t$, RPN generate $N$ proposals ${B_t=\{b_{t,n}\}}$ and corresponding objectness scores $S_t=\{s_{t,n}\}$ at each frame, where the index $n \in \{1,...,N\}$. Furthermore, we represent proposal features $F_t = \{f_{t,n}\}$ extracting from $B_t$.

\paragraph{\textit{Context aggregation in \modulenameshort{}.}} To mine the relationship between proposals from each frame, the attention-based operators~\cite{vaswani2017attention, wu2019sequence} are employed. Omitting time stamps, proposals from different frames are grouped to form $F^p = \cup_{t=1}^T F_t$. 
In our \modulenameshort{}, we devide $f^p_i \in F^p$ into $f^{cls}_i \in F^{cls}$ and $f^{loc}_i \in F^{loc}$, where $i$ is the index of proposals. 
To aggregate features $F^*=\{f^*_i\}$, where $* \in \{cls, loc\}$, in the following two independent paths, general attention-based operators are employed to reweight features from other proposals with learnable parameters.
The output of \modulenameshort{} ${F^{*'} = \{f^{*'}_i\}}$ can be computed as
% a learnable weighted sum of features from other proposals. 
% Given proposals ${B=\{b_i\}}$, objectness scores ${S=\{s_i\}}$ and features ${F^*=\{f^*_i\}}$ from all the frames, a general attention-based operator enhance features by a learnable weighted sum of features from other proposals. The ${F^{agg} = \{f^{agg}_i\}}$ can be computed as

\begin{equation}
    \begin{aligned}
        Q(F^*) &= W^*_q \cdot F^*, \\
        K(F^*) &= W^*_k \cdot F^*, \\
        Att(f^*_i, F^*) &= softmax(\frac{Q(f^*_i)K(F^*)^T}{\sqrt d^*}) F^*, \\
        f^{*'}_i &= f^*_i + Att(f^*_i, F^*),
    \end{aligned}
\end{equation}
where both $W^*_q \in \{W^{cls}_q, W^{loc}_q\}$ and $W^*_k \in \{W^{cls}_k, W^{loc}_k\}$ are individual linear learnable transformation matrices. $d^*$ is the dimension of $f^*_i \in F^*$.

\subsubsection{Path1: Aggregating the classification context and global feature of Proposals.}
\
\newline
The occluded or blurred objects in current frames may appear clearly in the neighbouring frames. And other objects in the scene can also help recognize the proposals. Hence, we firstly employ a Cls-Context Aggregation operator to augment features. Through operator simply captures the relationship between different proposals, however it lacks the ability acquire the global context of the entire video. Hence, we devote to study to extract and aggregate global context of the video.

\paragraph{Global context of frames.} Inspired by global context extraction in semantic segmentation~\cite{liu2015parsenet, zhao2017pyramid}, the global context of frames can be computed as

\begin{equation}
    \begin{aligned}
        G_{gcf}(\{M_t\}_{t=1}^T) &= Mean(\{M_t\}_{t=1}^T).
    \end{aligned}
    \label{eq:gcf}
\end{equation}

However, most of frames are with messy background, and objects only occupy a small region. Consequently, the extracted global context features contain limited knowledge about the objects.

% objects only occupy a small part the objects only occupy a small part of the entire video, and most of it is a messy background. As a result, the extracted global context only contains a small amount of global context about the objects in the frames.

\paragraph{Global context of proposals.}
In the test phase of faster-rcnn-style network, proposals mainly focus on the part of the scene where objects may exist and most of the background is filtered out. Therefore, feature extraction at proposal-level can better know the global context of objects in the video, which can be computed as
\begin{equation}
    G_{gcp}(F^{cls}) = Mean(F^{cls}).
    \label{eq:gcp}
\end{equation}
However, the proposals also contains some false negative cases. Even though these proposals include a part of the object, these information can not help to extract accurate global context due to bias. 

\paragraph{Highlight features from proposals within objects.}
To further expand the idea of extracting the global context of proposals, our approach is designed to emphasize high-quality proposal. Through observation, we find that proposals with high objectness scores produced by RPN mostly contains the main body or salient parts of the objects. And a large number of proposals can eliminate the uncertainty of the objectness scores for proposal quality evaluation. Specifically, we introduce the objectness score to weight different features corresponding to proposal, and in order to ensure the stability of the feature, we further normalize it, as follows:
\begin{equation}
    G_{hgcp}(F^{cls}) = \frac{\sum_i(s_i \times f^{cls}_i)}{\sum_i(s_i)}.
    \label{eq:hgcp}
\end{equation}
In order to synthesize Cls-Context aggregation and global feature of proposals, we calculate a set of factors from the output from equation~\ref{eq:hgcp} to selectively hightlight the class-dependet channels of aggregated features, as equation~\ref{eq:cls},
\begin{equation}
    f^{Video} = Softmax(NL(G_{hgcp}(F^{cls})))\cdot F^{cls'},
    \label{eq:cls}
\end{equation}
where $NL(\cdot)$ is non-linear transformations applied to the global context of proposals.

\subsubsection{Path2: Aggregating the localization context.}\
\newline
As previous analysis, the existing networks are employable to localize objects. However, to avoid the interference of too many contexts, we still adopt an independent Loc-Context Aggregation operator. The augmented $F^{loc'}$ can be trained only under the supervision of the annotated coordinates of bounding boxes.

\subsection{Sequence DIoU NMS}
\indent\paragraph{Sequence NMS.} Seq-NMS~\cite{han2016seq} is a classical post-processing for sequence detection. However,  
for objects that are dense and occlude each other in consecutive frames, Seq-NMS links the bounding boxes according to overlaps that will cause two different objects to be processed in a tubelet.
\paragraph{Action Tube and BLR.} Different from the thresholded linking criterion in ~\cite{han2016seq}, action tube~\cite{gkioxari2015finding} added overlaps into the optimization goal, which made the selecte sequence more smooth in space and had more opportunity to link the same objects in different frames. BLR~\cite{deng2019relation} further added the pair-wise relation weight from network into the optimization goal to process and optimize multiple frames at the same time, which also limited its application due to the necessary relation output.
\paragraph{DIoU NMS.} In fact, in image object detection, the false non-maximum suppression is also a problem still to be solved. DIoU NMS~\cite{zheng2020distance} is an extended overlap metric. Different from jaccard overlap, DIoU NMS considered the center distance of bounding boxes, which has better effect to distinguish crowded objects.
\paragraph{Our approach.} Note that since sequence selection is a key and difficult point in processing bounding boxes in frames, we improve the Seq-NMS with DIoU. Our post-processing operator can improve the performance significantly while maintaining the flexibility of origin methods, as shown in algrithms~\ref{alg:seq-dnms}.

\begin{algorithm}[htb] 
    \SetAlgoNoLine
    \caption{The algorithm of our Sequence DIoU NMS.} 
    \label{alg:seq-dnms} 
    \begin{algorithmic}[1] 
    \Require
    ${B_t=\{b_{t,n}\}}$,
    ${S_t=\{s_{t,n}\}}$,
    $\tau_1$, $\tau_2$
    \Statex$t \in \{1,...,T\}$ is the time stamp
    \Statex${B_t}$ is the list of initial bounding boxes in frame $t$
    \Statex${S_t}$ contains corresponding detection scores
    \Statex$\tau_1$ and $\tau_2$ are the threshold
    
    \Ensure optimal ${B_t=\{b_{t,n}\}}$, ${S_t=\{s_{t,n}\}}$
    \State Create linkes $L$:
    \Statex
    \For{$t=1;t \le T-1$}
    {
        $L_t = \Phi$

        \For{$b_i \in B_t$ and $b_j \in B_{t+1}$}
        {
            \If{$DIoU(b_i, b_j)\le \tau 1$}
            {
                $L_t \cup link(b_i,b_j)$
            }
        }
        $L \cup L_t$
    }
    \State Find maximum paths:
    \Statex
    find the maximum path $P = \{b_{t_0},...,b_{t_1}\}$ from $t_0$ to $t_1$,
    \Statex
    \While{$P \neq \Phi$ or $\sum\{s_{t_0},...,s_{t_1}\}$ or $L \neq \Phi$}
    {
        \For{$t=t_0;j \le t_1;$}
        {
            \For{$b_i \in B_t$}
            {
                \If{$DIoU(b_i, b_t)\le \tau_2$}
                {
                    delete $b_i$ and corresonding links;
                }
            }
        }
        update $L$
    }
    rescore the corresonding $\{s_{t_0},...,s_{t_1}\}$
    %\Return new ${B_t=\{b_t^i\}}$, ${S_t=\{s_t^i\}}$
    \end{algorithmic} 
    \end{algorithm}

\subsection{Relation to Other Approaches}
\
\indent\paragraph{Multi-head attention-based approaches.} In attention-based approaches~\cite{vaswani2017attention,deng2019relation}, the multi-head attention is used to make the attention operators to model different relations to enhance each proposals. In multi-head attention, the input features are splitted into different parts, which are calculated attention weight separately. Then the all of parts are enhanced correspondingly. 
Our approach differs significantly from these in operators and motivation. Although we also split the $f^{p}$ into two part, we use different supervision for each part, which reduce the contradiction between recognition and localization. And it needs to be emphasized that this split operator is a necessary pre-operation to extract global context of proposals.

\paragraph{Global Features Aggregation.} Global context has been proven effective in semantic segmentation~\cite{liu2015parsenet,zhao2017pyramid}, action recognition~\cite{wang2018videos} and similar tasks.
In semantic segmentation~\cite{liu2015parsenet,zhao2017pyramid,zhang2018context}, both foreground and background are densely encoded into the global context, without paying more attention to foreground objects.
action recognition~\cite{wang2018videos} can obviously benefit from the global context of the video. However, for the meaningless proposals produced by detectors, no processing methods have been proposed.
To the date of submission, we are the first to adopt and improve similar strategies to extract global context in video object detection. For the redundant and overlapping proposals in object detection pipeline, we disign a weighted aggregation strategy to obtain global context of proposal. Our approach can be trained in an end-to-end manner and adapted to most two-stage detectors.
